ECG-QA: A Comprehensive Question Answering Dataset Combined With Electrocardiogram

Question answering (QA) in the field of healthcare has received much attention due to significant advancements in natural language processing. However, existing healthcare QA datasets primarily focus on medical images, clinical notes, or structured electronic health record tables. This leaves the vast potential of combining electrocardiogram (ECG) data with these systems largely untapped. To address this gap, we present ECG-QA, the first QA dataset specifically designed for ECG analysis. The dataset comprises a total of 70 question templates that cover a wide range of clinically relevant ECG topics, each validated by an ECG expert to ensure their clinical utility. As a result, our dataset includes diverse ECG interpretation questions, including those that require a comparative analysis of two different ECGs. In addition, we have conducted numerous experiments to provide valuable insights for future research directions. We believe that ECG-QA will serve as a valuable resource for the development of intelligent QA systems capable of assisting clinicians in ECG interpretations. Dataset URL: https://github.com/Jwoo5/ecg-qa

==> tables/qa_qtype_p_result.tex <==
\begin{table}[ht]
    \caption{Performances for different question types \& attribute types where QA models were trained \& tested on the \textbf{paraphrased} version of the ECG-QA dataset.}
    \label{tab:qa_qtype_t_result}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{3}{*}{Question Type} & \multirow{3}{*}{\makecell{per Q-type\\majority}} & \multicolumn{2}{c}{M3AE} & \multicolumn{2}{c}{MedViLL} & \multicolumn{2}{c}{Transf.} & \multicolumn{2}{c}{Blind} & \multicolumn{2}{c}{Deaf} \\
        \cmidrule(r){3-12}
        & & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
        \midrule
        \textit{S-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{S-Choose} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{S-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{CC-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{CC-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{IC-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{IC-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & & \\
        \bottomrule
        \multicolumn{12}{l}{S: Single, CC: Consecutive-Comparison, IC: Irrelevant-Comparison}
    \end{tabular}
    }
\end{table}

==> tables/qa_qtype_t_result.tex <==
\begin{table}[ht]
    \caption{Performances for different question types \& attribute types where QA models were trained \& tested on the \textbf{template} version of the ECG-QA dataset.}
    % \label{tab:qa_qtype_t_result}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{3}{*}{Question Type} & \multirow{3}{*}{\makecell{per Q-type\\majority}} & \multicolumn{2}{c}{M3AE} & \multicolumn{2}{c}{MedViLL} & \multicolumn{2}{c}{Transf.} & \multicolumn{2}{c}{Blind} & \multicolumn{2}{c}{Deaf} \\
        \cmidrule(r){3-12}
        & & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
        \midrule
        \textit{S-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{S-Choose} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{S-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Noise & & & & & & & & & & &  \\
        Stage of infarction & & & & & & & & & & &  \\
        Extra systole & & & & & & & & & & &  \\
        Heart axis & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{CC-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{CC-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{IC-Verify} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & &  \\
        \midrule
        \textit{IC-Retrieve} & & & & & & & & & & &  \\
        SCP Code & & & & & & & & & & &  \\
        Numeric feature & & & & & & & & & & & \\
        \bottomrule
        \multicolumn{12}{l}{S: Single, CC: Consecutive-Comparison, IC: Irrelevant-Comparison}
    \end{tabular}
    }
\end{table}

==> tables/qa_t_result.tex <==
\begin{table}[ht]
    \caption{Test performances for different question types where QA models were trained \& tested on the \textbf{template} version of the ECG-QA dataset.}
    \label{tab:qa_t_result}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{3}{*}{Question Type} & \multirow{3}{*}{\makecell{per Q-type\\majority}} & \multicolumn{2}{c}{M3AE} & \multicolumn{2}{c}{MedViLL} & \multicolumn{2}{c}{Transf.} & \multicolumn{2}{c}{Blind Transf.} & \multicolumn{2}{c}{Deaf Transf.} \\
        \cmidrule(r){3-12}
        & & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
        \midrule
        S-Verify & $67.73$ & $75.36$ & $0.7773$ & $\bf75.38$ & $\bf0.7864$ & $72.70$ & $0.7255$ & $ $ & $ $ & $ $ & $ $ \\
        S-Choose & $31.15$ & $\bf55.90$ & $\bf0.8423$ & $53.75$ & $0.8416$ & $46.07$ & $0.7980$ & $ $ & $ $ & $ $ & $ $ \\
        S-Retrieve & $23.66$ & $\bf41.72$ & $0.8363$ & $41.28$ & $\bf0.8471$ & $38.44$ & $0.7942$ & $ $ & $ $ & $ $ & $ $ \\
        CC-Verify & $62.81$ & $75.83$ & $0.8042$ & $\bf76.46$ & $\bf0.8112$ & $71.69$ & $0.7624$ & $ $ & $ $ & $ $ & $ $ \\
        CC-Retrieve & $17.32$ & $19.31$ & $0.8036$ & $\bf23.77$ & $\bf0.8290$ & $19.88$ & $0.7881$ & $ $ & $ $ & $ $ & $ $ \\
        IC-Verify & $66.11$ & $75.36$ & $0.7842$ & $\bf77.62$ & $\bf0.8249$ & $68.43$ & $0.7318$ & $ $ & $ $ & $ $ & $ $ \\
        IC-Retrieve & $1.10$ & $\bf5.23$ & $0.7562$ & $4.34$ & $\bf0.7954$ & $2.97$ & $0.7463$ & $ $ & $ $ & $ $ & $ $ \\
        \bottomrule
        \multicolumn{12}{l}{S: Single, CC: Consecutive-Comparison, IC: Irrelevant-Comparison}
    \end{tabular}
    }
\end{table}

==> tables/sup_template2.tex <==
\begin{table}[t]
    \caption{Full list of question templates (Continued).}
    \label{tab:sup_template2}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccl}
        \toprule
        ID & Question Type & Attribute Type & \multicolumn{1}{c}{Template} \\
        \midrule
        49 & CC-Query & SCP code & \makecell[l]{What symptoms still remain in the recent tracing as compared to the previous one?} \\
        \cmidrule{1-4}
        50 & CC-Verify & Numeric feature & \makecell[l]{Compared to the previous tracing, has the \texttt{\$\{numeric\_feature\}} of the recent tracing \\ become normal?} \\
        \cmidrule{1-4}
        51 & CC-Verify & Numeric feature & \makecell[l]{Compared to the previous tracing, has the \texttt{\$\{numeric\_feature\}} of the recent tracing \\ changed to an abnormal value?} \\
        \cmidrule{1-4}
        52 & CC-Verify & Numeric feature & \makecell[l]{Compared to the previous tracing, does the \texttt{\$\{numeric\_feature\}} still show an \\ abnormal value in the recent tracing?} \\
        \cmidrule{1-4}
        53 & CC-Verify & Numeric feature & \makecell[l]{Compared to the previous tracing, is the \texttt{\$\{numeric\_feature\}} still considered \\ normal in the recent tracing?} \\
        \cmidrule{1-4}
        54 & CC-Query & Numeric feature & \makecell[l]{What numeric features of the recent tracing now have become normal compared to \\ the previous one?} \\
        \cmidrule{1-4}
        55 & CC-Query & Numeric feature & \makecell[l]{What numeric features of the recent tracing are now considered abnormal values \\ compared to the previous one?} \\
        \cmidrule{1-4}
        56 & CC-Query & Numeric feature & \makecell[l]{What numeric features of the recent tracing are still abnormal compared to \\ the previous one?} \\
        \cmidrule{1-4}
        57 & CI-Verify & SCP code & \makecell[l]{Compared to the first ECG, has \texttt{\$\{scp\_code\}} been resolved in the second ECG?} \\
        \cmidrule{1-4}
        58 & CI-Verify & SCP code & \makecell[l]{Compared to the first ECG, has \texttt{\$\{scp\_code\}} been newly detected in the second ECG?} \\
        \cmidrule{1-4}
        59 & CI-Verify & SCP code & \makecell[l]{Compared to the first ECG, does \texttt{\$\{scp\_code\}} still remain in the second ECG?} \\
        \cmidrule{1-4}
        60 & CI-Verify & SCP code & \makecell[l]{Compared to the first ECG, is \texttt{\$\{scp\_code\}} still not found in the second ECG?} \\
        \cmidrule{1-4}
        61 & CI-Query & SCP code & \makecell[l]{What symptoms have been resolved in the second ECG as compared to the first ECG?} \\
        \cmidrule{1-4}
        62 & CI-Query & SCP code & \makecell[l]{What symptoms are newly detected in the second ECG as compared to the first ECG?} \\
        \cmidrule{1-4}
        63 & CI-Query & SCP code & \makecell[l]{What symptoms still remain in the second ECG as compared to the first ECG?} \\
        \cmidrule{1-4}
        64 & CI-Verify & Numeric feature & \makecell[l]{Compared to the first ECG, has the \texttt{\$\{numeric\_feature\}} of the second ECG become \\ normal?} \\
        \cmidrule{1-4}
        65 & CI-Verify & Numeric feature & \makecell[l]{Compared to the first ECG, has the \texttt{\$\{numeirc\_feature\}} of the second ECG changed \\ to an abnormal value?} \\
        \cmidrule{1-4}
        66 & CI-Verify & Numeric feature & \makecell[l]{Compared to the first ECG, does the \texttt{\$\{numeric\_feature\}} still show an abnormal \\ value in the second ECG?} \\
        \cmidrule{1-4}
        67 & CI-Verify & Numeric feature & \makecell[l]{Compared to the first ECG, is the \texttt{\$\{numeric\_feature\}} still normal in the second ECG?} \\
        \cmidrule{1-4}
        68 & CI-Query & Numeric feature & \makecell[l]{What numeric features of the second ECG now have become normal as compared to the \\ first ECG?} \\
        \cmidrule{1-4}
        69 & CI-Query & Numeric feature & \makecell[l]{What numeric features of the second ECG are now considered abnormal values as \\ compared to the first ECG?} \\
        \cmidrule{1-4}
        70 & CI-Query & Numeric feature & \makecell[l]{What numeric features of the second ECG are still abnormal as compared to the first ECG?} \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/sup_upper_attr_result_joint.tex <==
\begin{table}[htbp]
    \captionsetup{font={small}}
    \caption{Test performances of QA baselines \& upper bound models for different attributes in \textbf{Single-Verify} questions.
    For the convenience of comparison, we selected SE-WRN~\cite{han2021towards} and MAX for the upper bound models, and M$^3$AE$^\dagger$~\cite{chen2022multi} for the QA baseline.
    Attributes are sorted in alphabetical order.
    We provide 95\% confidence interval across 3 random seeds.
    }
    \label{tab:sup_upper_attr_result_joint}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \multicolumn{1}{c}{\multirow{3}{*}{Attribute name}} & \multicolumn{2}{c}{SE-WRN~\cite{han2021towards}} & \multicolumn{2}{c}{MAX} & \multicolumn{2}{c}{M$^3$AE$^\dagger$~\cite{chen2022multi}} \\
        \cmidrule(r){2-7}
        & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
        \midrule
        Abnormal qrs & $71.7_{ \pm 3.3 }$ & $0.734_{ \pm 0.046 }$ & $73.3_{ \pm 1.9 }$ & $0.779_{ \pm 0.033 }$ & $76.7_{ \pm 1.9 }$ & $0.791_{ \pm 0.036 }$ \\
        Above the normal range of p duration & $86.7_{ \pm 0.0 }$ & $0.939_{ \pm 0.014 }$ & $88.3_{ \pm 3.3 }$ & $0.948_{ \pm 0.018 }$ & $67.8_{ \pm 6.1 }$ & $0.683_{ \pm 0.030 }$ \\
        Above the normal range of pr interval & $91.1_{ \pm 2.2 }$ & $0.973_{ \pm 0.015 }$ & $91.1_{ \pm 2.2 }$ & $0.976_{ \pm 0.010 }$ & $86.7_{ \pm 3.8 }$ & $0.893_{ \pm 0.046 }$ \\
        Above the normal range of qrs duration & $87.8_{ \pm 2.9 }$ & $0.932_{ \pm 0.007 }$ & $89.4_{ \pm 1.1 }$ & $0.958_{ \pm 0.002 }$ & $86.7_{ \pm 5.0 }$ & $0.901_{ \pm 0.073 }$ \\
        Above the normal range of qt corrected & $76.1_{ \pm 2.9 }$ & $0.862_{ \pm 0.010 }$ & $77.2_{ \pm 1.1 }$ & $0.862_{ \pm 0.010 }$ & $76.1_{ \pm 2.2 }$ & $0.763_{ \pm 0.060 }$ \\
        Above the normal range of qt interval & $85.0_{ \pm 5.7 }$ & $0.940_{ \pm 0.038 }$ & $90.6_{ \pm 2.9 }$ & $0.966_{ \pm 0.011 }$ & $81.1_{ \pm 1.1 }$ & $0.824_{ \pm 0.060 }$ \\
        Above the normal range of rr interval & $97.2_{ \pm 1.1 }$ & $0.999_{ \pm 0.001 }$ & $98.9_{ \pm 1.1 }$ & $1.000_{ \pm 0.000 }$ & $98.3_{ \pm 1.9 }$ & $0.992_{ \pm 0.017 }$ \\
        Any diagnostic symptoms & $81.7_{ \pm 3.3 }$ & $0.865_{ \pm 0.043 }$ & $85.6_{ \pm 2.2 }$ & $0.914_{ \pm 0.012 }$ & $88.6_{ \pm 1.1 }$ & $0.918_{ \pm 0.006 }$ \\
        Any form-related symptoms & $74.4_{ \pm 3.9 }$ & $0.746_{ \pm 0.031 }$ & $81.1_{ \pm 4.4 }$ & $0.820_{ \pm 0.023 }$ & $78.9_{ \pm 6.1 }$ & $0.820_{ \pm 0.045 }$ \\
        Any kind of abnormal symptoms & $81.7_{ \pm 1.9 }$ & $0.864_{ \pm 0.011 }$ & $82.8_{ \pm 3.9 }$ & $0.877_{ \pm 0.030 }$ & $74.5_{ \pm 12.6 }$ & $0.710_{ \pm 0.138 }$ \\
        Any kind of extra systoles & $85.3_{ \pm 5.7 }$ & $0.874_{ \pm 0.035 }$ & $94.7_{ \pm 1.3 }$ & $0.960_{ \pm 0.020 }$ & $92.0_{ \pm 3.9 }$ & $0.932_{ \pm 0.047 }$ \\
        Any kind of noises & $70.9_{ \pm 0.8 }$ & $0.755_{ \pm 0.003 }$ & $74.0_{ \pm 0.8 }$ & $0.779_{ \pm 0.008 }$ & $68.0_{ \pm 1.5 }$ & $0.612_{ \pm 0.018 }$ \\
        Any rhythm-related symptoms & $83.9_{ \pm 4.7 }$ & $0.882_{ \pm 0.043 }$ & $85.6_{ \pm 5.4 }$ & $0.891_{ \pm 0.038 }$ & $70.5_{ \pm 2.2 }$ & $0.738_{ \pm 0.032 }$ \\
        Atrial fibrillation & $87.2_{ \pm 2.9 }$ & $0.954_{ \pm 0.002 }$ & $94.4_{ \pm 1.1 }$ & $0.961_{ \pm 0.010 }$ & $92.2_{ \pm 1.1 }$ & $0.931_{ \pm 0.019 }$ \\
        Atrial flutter & $94.4_{ \pm 0.0 }$ & $0.987_{ \pm 0.020 }$ & $94.4_{ \pm 0.0 }$ & $0.991_{ \pm 0.013 }$ & $97.2_{ \pm 0.0 }$ & $0.945_{ \pm 0.020 }$ \\
        Atrial premature complex & $82.2_{ \pm 2.2 }$ & $0.901_{ \pm 0.038 }$ & $83.9_{ \pm 3.9 }$ & $0.950_{ \pm 0.023 }$ & $82.8_{ \pm 5.8 }$ & $0.861_{ \pm 0.048 }$ \\
        Baseline drift & $80.5_{ \pm 1.0 }$ & $0.889_{ \pm 0.003 }$ & $80.5_{ \pm 1.0 }$ & $0.889_{ \pm 0.003 }$ & $69.2_{ \pm 1.2 }$ & $0.664_{ \pm 0.006 }$ \\
        Below the normal range of pr interval & $91.1_{ \pm 3.9 }$ & $0.951_{ \pm 0.025 }$ & $92.8_{ \pm 2.9 }$ & $0.968_{ \pm 0.008 }$ & $77.8_{ \pm 6.1 }$ & $0.811_{ \pm 0.018 }$ \\
        Below the normal range of qrs duration & $91.7_{ \pm 3.8 }$ & $0.989_{ \pm 0.006 }$ & $92.2_{ \pm 2.9 }$ & $0.995_{ \pm 0.005 }$ & $88.9_{ \pm 1.1 }$ & $0.876_{ \pm 0.014 }$ \\
        Below the normal range of qt corrected & $86.1_{ \pm 2.9 }$ & $0.973_{ \pm 0.011 }$ & $92.2_{ \pm 1.1 }$ & $0.988_{ \pm 0.010 }$ & $86.7_{ \pm 3.8 }$ & $0.912_{ \pm 0.036 }$ \\
        Below the normal range of qt interval & $83.9_{ \pm 3.9 }$ & $0.940_{ \pm 0.026 }$ & $87.8_{ \pm 1.1 }$ & $0.954_{ \pm 0.004 }$ & $76.1_{ \pm 2.9 }$ & $0.809_{ \pm 0.030 }$ \\
        Below the normal range of rr interval & $100.0_{ \pm 0.0 }$ & $1.000_{ \pm 0.000 }$ & $100.0_{ \pm 0.0 }$ & $1.000_{ \pm 0.000 }$ & $97.2_{ \pm 1.1 }$ & $0.982_{ \pm 0.004 }$ \\
        Bigeminal pattern (unknown origin, supraventricular, or ventricular) & $85.3_{ \pm 4.7 }$ & $0.853_{ \pm 0.078 }$ & $87.3_{ \pm 2.6 }$ & $0.912_{ \pm 0.057 }$ & $88.0_{ \pm 2.3 }$ & $0.862_{ \pm 0.021 }$ \\
        Burst noise & $67.9_{ \pm 0.4 }$ & $0.697_{ \pm 0.056 }$ & $75.5_{ \pm 0.7 }$ & $0.761_{ \pm 0.023 }$ & $66.6_{ \pm 0.2 }$ & $0.523_{ \pm 0.033 }$ \\
        Complete left bundle branch block & $94.4_{ \pm 1.1 }$ & $0.992_{ \pm 0.003 }$ & $96.1_{ \pm 2.2 }$ & $0.994_{ \pm 0.003 }$ & $95.0_{ \pm 0.0 }$ & $0.976_{ \pm 0.016 }$ \\
        Complete right bundle branch block & $97.2_{ \pm 1.1 }$ & $0.998_{ \pm 0.003 }$ & $98.9_{ \pm 1.1 }$ & $1.000_{ \pm 0.000 }$ & $97.3_{ \pm 1.1 }$ & $0.984_{ \pm 0.026 }$ \\
        Conduction disturbance & $86.1_{ \pm 2.2 }$ & $0.938_{ \pm 0.016 }$ & $90.0_{ \pm 0.0 }$ & $0.952_{ \pm 0.006 }$ & $91.1_{ \pm 5.4 }$ & $0.933_{ \pm 0.032 }$ \\
        Digitalis effect & $83.6_{ \pm 1.1 }$ & $0.947_{ \pm 0.019 }$ & $83.6_{ \pm 1.1 }$ & $0.953_{ \pm 0.013 }$ & $69.2_{ \pm 5.2 }$ & $0.827_{ \pm 0.014 }$ \\
        Early stage of myocardial infarction & $78.0_{ \pm 3.3 }$ & $0.864_{ \pm 0.023 }$ & $80.8_{ \pm 2.9 }$ & $0.889_{ \pm 0.008 }$ & $86.3_{ \pm 1.9 }$ & $0.877_{ \pm 0.024 }$ \\
        Electrodes problems & $81.3_{ \pm 1.0 }$ & $0.720_{ \pm 0.069 }$ & $83.8_{ \pm 1.0 }$ & $0.732_{ \pm 0.061 }$ & $84.3_{ \pm 1.0 }$ & $0.599_{ \pm 0.051 }$ \\
        Extrasystoles & $86.1_{ \pm 2.9 }$ & $0.915_{ \pm 0.043 }$ & $90.6_{ \pm 2.2 }$ & $0.953_{ \pm 0.051 }$ & $92.2_{ \pm 2.9 }$ & $0.935_{ \pm 0.020 }$ \\
        Extreme axis deviation & $90.1_{ \pm 5.0 }$ & $0.953_{ \pm 0.018 }$ & $91.8_{ \pm 3.0 }$ & $0.960_{ \pm 0.009 }$ & $90.1_{ \pm 3.0 }$ & $0.913_{ \pm 0.028 }$ \\
        First degree av block & $85.0_{ \pm 3.3 }$ & $0.913_{ \pm 0.011 }$ & $88.3_{ \pm 3.3 }$ & $0.947_{ \pm 0.015 }$ & $83.6_{ \pm 2.7 }$ & $0.861_{ \pm 0.029 }$ \\
        High qrs voltage & $78.9_{ \pm 2.0 }$ & $0.705_{ \pm 0.020 }$ & $80.7_{ \pm 0.8 }$ & $0.726_{ \pm 0.040 }$ & $79.3_{ \pm 0.0 }$ & $0.602_{ \pm 0.082 }$ \\
        Hypertrophy & $80.6_{ \pm 4.7 }$ & $0.870_{ \pm 0.032 }$ & $83.3_{ \pm 1.9 }$ & $0.889_{ \pm 0.014 }$ & $72.8_{ \pm 2.9 }$ & $0.765_{ \pm 0.027 }$ \\
        Incomplete left bundle branch block & $81.0_{ \pm 1.3 }$ & $0.954_{ \pm 0.018 }$ & $81.7_{ \pm 1.3 }$ & $0.954_{ \pm 0.018 }$ & $86.3_{ \pm 0.0 }$ & $0.878_{ \pm 0.034 }$ \\
        Incomplete right bundle branch block & $73.9_{ \pm 2.9 }$ & $0.843_{ \pm 0.050 }$ & $78.3_{ \pm 3.3 }$ & $0.905_{ \pm 0.012 }$ & $69.6_{ \pm 2.8 }$ & $0.808_{ \pm 0.024 }$ \\
        Inverted t-waves & $87.3_{ \pm 0.5 }$ & $0.949_{ \pm 0.006 }$ & $87.3_{ \pm 0.5 }$ & $0.950_{ \pm 0.005 }$ & $75.2_{ \pm 1.7 }$ & $0.769_{ \pm 0.016 }$ \\
        Ischemic & $71.3_{ \pm 0.8 }$ & $0.835_{ \pm 0.017 }$ & $72.1_{ \pm 0.9 }$ & $0.835_{ \pm 0.017 }$ & $67.4_{ \pm 1.3 }$ & $0.722_{ \pm 0.015 }$ \\
        Late stage of myocardial infarction & $85.0_{ \pm 1.3 }$ & $0.681_{ \pm 0.055 }$ & $85.0_{ \pm 1.3 }$ & $0.699_{ \pm 0.034 }$ & $83.7_{ \pm 2.3 }$ & $0.777_{ \pm 0.046 }$ \\
        Left anterior fascicular block & $98.3_{ \pm 1.9 }$ & $0.995_{ \pm 0.005 }$ & $98.9_{ \pm 1.1 }$ & $1.000_{ \pm 0.000 }$ & $84.3_{ \pm 1.0 }$ & $0.935_{ \pm 0.008 }$ \\
        Left atrial overload/enlargement & $70.6_{ \pm 2.2 }$ & $0.762_{ \pm 0.033 }$ & $71.1_{ \pm 1.1 }$ & $0.780_{ \pm 0.034 }$ & $52.1_{ \pm 6.7 }$ & $0.618_{ \pm 0.036 }$ \\
        Left axis deviation & $87.8_{ \pm 2.2 }$ & $0.951_{ \pm 0.026 }$ & $88.9_{ \pm 2.2 }$ & $0.953_{ \pm 0.023 }$ & $82.8_{ \pm 5.8 }$ & $0.902_{ \pm 0.050 }$ \\
        Left posterior fascicular block & $84.4_{ \pm 1.1 }$ & $0.996_{ \pm 0.004 }$ & $84.4_{ \pm 1.1 }$ & $0.996_{ \pm 0.004 }$ & $92.8_{ \pm 2.9 }$ & $0.942_{ \pm 0.019 }$ \\
        Left ventricular hypertrophy & $88.3_{ \pm 1.9 }$ & $0.969_{ \pm 0.016 }$ & $88.9_{ \pm 1.1 }$ & $0.973_{ \pm 0.009 }$ & $62.1_{ \pm 4.3 }$ & $0.734_{ \pm 0.025 }$ \\
        Long qt-interval & $78.4_{ \pm 0.0 }$ & $0.842_{ \pm 0.061 }$ & $78.4_{ \pm 0.0 }$ & $0.842_{ \pm 0.061 }$ & $78.8_{ \pm 2.2 }$ & $0.562_{ \pm 0.138 }$ \\
        Low amplitude t-wave & $74.5_{ \pm 1.1 }$ & $0.858_{ \pm 0.004 }$ & $74.5_{ \pm 1.1 }$ & $0.858_{ \pm 0.004 }$ & $73.9_{ \pm 3.1 }$ & $0.728_{ \pm 0.026 }$ \\
        Low qrs voltages in the frontal and horizontal leads & $75.7_{ \pm 1.4 }$ & $0.850_{ \pm 0.015 }$ & $76.5_{ \pm 1.0 }$ & $0.863_{ \pm 0.018 }$ & $69.8_{ \pm 0.9 }$ & $0.650_{ \pm 0.056 }$ \\
        Middle stage of myocardial infarction & $68.9_{ \pm 2.9 }$ & $0.762_{ \pm 0.034 }$ & $76.1_{ \pm 2.2 }$ & $0.821_{ \pm 0.027 }$ & $75.0_{ \pm 1.9 }$ & $0.817_{ \pm 0.020 }$ \\
        Myocardial infarction & $77.5_{ \pm 1.2 }$ & $0.844_{ \pm 0.007 }$ & $80.2_{ \pm 1.1 }$ & $0.873_{ \pm 0.014 }$ & $71.1_{ \pm 0.8 }$ & $0.800_{ \pm 0.005 }$ \\
        Non-diagnostic t abnormalities & $76.1_{ \pm 0.8 }$ & $0.841_{ \pm 0.003 }$ & $76.1_{ \pm 0.8 }$ & $0.841_{ \pm 0.003 }$ & $70.7_{ \pm 1.6 }$ & $0.778_{ \pm 0.040 }$ \\
        Non-specific intraventricular conduction disturbance (block) & $68.3_{ \pm 3.3 }$ & $0.620_{ \pm 0.043 }$ & $71.7_{ \pm 0.0 }$ & $0.819_{ \pm 0.027 }$ & $71.4_{ \pm 3.1 }$ & $0.674_{ \pm 0.059 }$ \\
        Non-specific ischemic & $83.9_{ \pm 3.9 }$ & $0.947_{ \pm 0.026 }$ & $85.6_{ \pm 1.1 }$ & $0.957_{ \pm 0.013 }$ & $70.8_{ \pm 1.6 }$ & $0.837_{ \pm 0.006 }$ \\
        Non-specific st changes & $77.7_{ \pm 0.3 }$ & $0.788_{ \pm 0.023 }$ & $78.2_{ \pm 0.4 }$ & $0.788_{ \pm 0.023 }$ & $76.9_{ \pm 0.6 }$ & $0.683_{ \pm 0.025 }$ \\
        Non-specific st depression & $84.6_{ \pm 0.7 }$ & $0.918_{ \pm 0.006 }$ & $84.9_{ \pm 0.4 }$ & $0.918_{ \pm 0.006 }$ & $71.7_{ \pm 1.4 }$ & $0.706_{ \pm 0.018 }$ \\
        Non-specific st elevation & $83.3_{ \pm 0.0 }$ & $0.713_{ \pm 0.171 }$ & $83.3_{ \pm 0.0 }$ & $0.850_{ \pm 0.112 }$ & $83.3_{ \pm 0.0 }$ & $0.583_{ \pm 0.059 }$ \\
        Non-specific t-wave changes & $77.4_{ \pm 1.2 }$ & $0.850_{ \pm 0.011 }$ & $77.4_{ \pm 1.2 }$ & $0.850_{ \pm 0.011 }$ & $71.9_{ \pm 1.2 }$ & $0.688_{ \pm 0.045 }$ \\
        Normal ecg & $80.6_{ \pm 3.9 }$ & $0.864_{ \pm 0.050 }$ & $82.8_{ \pm 2.9 }$ & $0.918_{ \pm 0.010 }$ & $72.2_{ \pm 4.7 }$ & $0.819_{ \pm 0.021 }$ \\
        Normal functioning artificial pacemaker & $97.2_{ \pm 1.4 }$ & $0.997_{ \pm 0.006 }$ & $100.0_{ \pm 0.0 }$ & $1.000_{ \pm 0.000 }$ & $98.6_{ \pm 2.7 }$ & $0.997_{ \pm 0.006 }$ \\
        Normal heart axis & $95.6_{ \pm 2.2 }$ & $0.992_{ \pm 0.009 }$ & $96.1_{ \pm 1.1 }$ & $0.997_{ \pm 0.001 }$ & $93.9_{ \pm 2.2 }$ & $0.981_{ \pm 0.019 }$ \\
        Prolonged pr interval & $86.1_{ \pm 2.9 }$ & $0.988_{ \pm 0.012 }$ & $90.6_{ \pm 1.1 }$ & $0.992_{ \pm 0.013 }$ & $91.7_{ \pm 5.7 }$ & $0.920_{ \pm 0.027 }$ \\
        Q waves present & $83.4_{ \pm 2.2 }$ & $0.911_{ \pm 0.005 }$ & $84.3_{ \pm 0.5 }$ & $0.911_{ \pm 0.005 }$ & $73.9_{ \pm 0.5 }$ & $0.685_{ \pm 0.012 }$ \\
        Right atrial overload/enlargement & $84.5_{ \pm 4.7 }$ & $0.979_{ \pm 0.008 }$ & $84.5_{ \pm 4.7 }$ & $0.979_{ \pm 0.008 }$ & $82.2_{ \pm 2.3 }$ & $0.764_{ \pm 0.075 }$ \\
        Right axis deviation & $91.1_{ \pm 1.1 }$ & $0.959_{ \pm 0.027 }$ & $92.8_{ \pm 1.1 }$ & $0.971_{ \pm 0.009 }$ & $91.1_{ \pm 2.9 }$ & $0.957_{ \pm 0.018 }$ \\
        Sinus arrhythmia & $78.9_{ \pm 4.7 }$ & $0.795_{ \pm 0.097 }$ & $80.6_{ \pm 2.9 }$ & $0.869_{ \pm 0.038 }$ & $81.7_{ \pm 7.5 }$ & $0.835_{ \pm 0.060 }$ \\
        Sinus bradycardia & $87.8_{ \pm 1.1 }$ & $0.960_{ \pm 0.018 }$ & $89.4_{ \pm 2.2 }$ & $0.965_{ \pm 0.009 }$ & $85.6_{ \pm 4.7 }$ & $0.882_{ \pm 0.050 }$ \\
        Sinus rhythm & $78.3_{ \pm 5.0 }$ & $0.848_{ \pm 0.024 }$ & $81.1_{ \pm 4.4 }$ & $0.864_{ \pm 0.018 }$ & $71.1_{ \pm 2.9 }$ & $0.786_{ \pm 0.035 }$ \\
        Sinus tachycardia & $95.0_{ \pm 1.9 }$ & $0.990_{ \pm 0.006 }$ & $97.2_{ \pm 1.1 }$ & $0.996_{ \pm 0.004 }$ & $96.1_{ \pm 2.2 }$ & $0.987_{ \pm 0.000 }$ \\
        St/t change & $78.9_{ \pm 1.1 }$ & $0.833_{ \pm 0.022 }$ & $81.1_{ \pm 2.2 }$ & $0.868_{ \pm 0.008 }$ & $79.5_{ \pm 2.9 }$ & $0.831_{ \pm 0.019 }$ \\
        Static noise & $71.1_{ \pm 1.1 }$ & $0.736_{ \pm 0.014 }$ & $71.1_{ \pm 1.1 }$ & $0.736_{ \pm 0.014 }$ & $66.7_{ \pm 0.5 }$ & $0.580_{ \pm 0.010 }$ \\
        Subendocardial injury & $75.4_{ \pm 2.1 }$ & $0.968_{ \pm 0.006 }$ & $77.9_{ \pm 0.5 }$ & $0.969_{ \pm 0.007 }$ & $86.2_{ \pm 0.9 }$ & $0.903_{ \pm 0.019 }$ \\
        Supraventricular extrasystoles & $83.3_{ \pm 3.8 }$ & $0.838_{ \pm 0.032 }$ & $86.1_{ \pm 2.9 }$ & $0.883_{ \pm 0.012 }$ & $85.0_{ \pm 1.9 }$ & $0.845_{ \pm 0.015 }$ \\
        Supraventricular tachycardia & $92.6_{ \pm 3.6 }$ & $0.941_{ \pm 0.077 }$ & $92.6_{ \pm 3.6 }$ & $0.963_{ \pm 0.073 }$ & $94.4_{ \pm 0.0 }$ & $0.876_{ \pm 0.069 }$ \\
        T-wave abnormality & $83.3_{ \pm 0.0 }$ & $0.461_{ \pm 0.107 }$ & $83.3_{ \pm 0.0 }$ & $0.532_{ \pm 0.024 }$ & $83.5_{ \pm 0.4 }$ & $0.498_{ \pm 0.088 }$ \\
        Ventricular extrasystoles & $79.4_{ \pm 2.9 }$ & $0.894_{ \pm 0.034 }$ & $81.1_{ \pm 1.1 }$ & $0.910_{ \pm 0.027 }$ & $86.1_{ \pm 2.9 }$ & $0.878_{ \pm 0.028 }$ \\
        Ventricular premature complex & $91.1_{ \pm 1.1 }$ & $0.974_{ \pm 0.009 }$ & $93.3_{ \pm 1.9 }$ & $0.978_{ \pm 0.004 }$ & $95.0_{ \pm 1.9 }$ & $0.956_{ \pm 0.010 }$ \\
        Voltage criteria (qrs) for left ventricular hypertrophy & $82.6_{ \pm 1.9 }$ & $0.898_{ \pm 0.027 }$ & $82.6_{ \pm 1.9 }$ & $0.912_{ \pm 0.022 }$ & $69.6_{ \pm 1.5 }$ & $0.655_{ \pm 0.029 }$ \\
        Within the normal range of p duration & $76.1_{ \pm 2.9 }$ & $0.875_{ \pm 0.032 }$ & $85.0_{ \pm 5.0 }$ & $0.948_{ \pm 0.027 }$ & $67.8_{ \pm 7.1 }$ & $0.691_{ \pm 0.050 }$ \\
        Within the normal range of pr interval & $79.4_{ \pm 2.9 }$ & $0.876_{ \pm 0.009 }$ & $85.0_{ \pm 1.9 }$ & $0.916_{ \pm 0.011 }$ & $71.1_{ \pm 4.4 }$ & $0.739_{ \pm 0.033 }$ \\
        Within the normal range of qrs duration & $81.1_{ \pm 2.2 }$ & $0.889_{ \pm 0.015 }$ & $83.3_{ \pm 5.0 }$ & $0.925_{ \pm 0.045 }$ & $76.7_{ \pm 5.0 }$ & $0.792_{ \pm 0.029 }$ \\
        Within the normal range of qt corrected & $76.7_{ \pm 8.6 }$ & $0.873_{ \pm 0.057 }$ & $82.8_{ \pm 4.4 }$ & $0.903_{ \pm 0.024 }$ & $78.9_{ \pm 3.9 }$ & $0.811_{ \pm 0.013 }$ \\
        Within the normal range of qt interval & $78.3_{ \pm 5.7 }$ & $0.876_{ \pm 0.023 }$ & $85.6_{ \pm 3.9 }$ & $0.922_{ \pm 0.026 }$ & $81.3_{ \pm 7.0 }$ & $0.834_{ \pm 0.063 }$ \\
        Within the normal range of rr interval & $88.9_{ \pm 3.9 }$ & $0.962_{ \pm 0.020 }$ & $96.7_{ \pm 1.9 }$ & $0.997_{ \pm 0.004 }$ & $96.1_{ \pm 1.1 }$ & $0.978_{ \pm 0.016 }$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/upperbound_result_attr.tex <==
\begin{table}[ht]
    \caption{Macro-averaged test performances over 83 attributes for \textbf{Single-Verify} questions}
    \label{tab:upper_attr}
    \centering
    \begin{tabular}{lcc}
        \toprule
        & Accuracy & AUROC \\
        \midrule
        \textit{QA Models} & & \\
        M3AE$_{template}$ & $80.70$ & $0.8230$  \\
        M3AE$_{paraphrased}$ & $80.81$ & $0.8083$ \\
        MedViLL$_{template}$ & $81.18$ & $0.8197$ \\
        MedViLL$_{paraphrased}$ & $79.76$ & $0.8088$ \\
        Transformer$_{template}$ & $76.99$ & $0.7770$ \\
        Transformer$_{paraphrased}$ & $76.39$ & $0.7644$ \\
        \midrule
        \multicolumn{3}{l}{\textit{Upper bound Models}}\\
        W2V+CMSC+RLM~\cite{oh2022lead} & $82.98$ & $0.8643$ \\
        Resnet-Attention~\cite{nejedly2021classification} & $82.56$ & $0.8750$  \\
        SE-WRN~\cite{han2021towards} & $83.09$ & $0.8826$ \\
        MAX & $85.40$ & $0.9066$ \\
        % \midrule
        % \multicolumn{3}{l}{\textit{Classification Models Trained on the Independent Dataset}} \\
        % W2V+CMSC+RLM~\cite{oh2022lead} & $84.92$ & $0.9076$ \\
        % Resnet-Attention~\cite{nejedly2021classification} & $84.53$ & $0.9066$ \\
        % SE-WRN~\cite{han2021towards} & $84.27$ & $0.9035$ \\
        % MAX & $87.30$ & $0.9262$ \\
        \bottomrule
    \end{tabular}
\end{table}
